The Peano software - parallel, automaton-based, dynamically adaptive grid traversals

We discuss the design decisions, design alternatives and rationale behind the third generation of Peano, a framework for dynamically adaptive Cartesian meshes derived from spacetrees. Peano ties the mesh traversal to the mesh storage and supports only one element-wise traversal order resulting from space-filling curves. The user is not free to choose a traversal order herself. The traversal can exploit regular grid subregions and shared memory as well as distributed memory systems with almost no modifications to a serial application code. We formalize the software design by means of two interacting automata---one automaton for the multiscale grid traversal and one for the application-specific algorithmic steps. This yields a callback-based programming paradigm. We further sketch the supported application types and the two data storage schemes realized, before we detail high-performance computing aspects and lessons learned. Special emphasis is put on observations regarding the used programming idioms and algorithmic concepts. This transforms our report from a "one way to implement things" code description into a generic discussion and summary of some alternatives, rationale and design decisions to be made for any tree-based adaptive mesh refinement software.

==> a3_experimental-setups.tex <==
\section{Rationale of experimental setups}

 
Throughout our experiments working with grids illustrated in Figure
\ref{figure:results} we use six Peano instances holding 2, 11, 28, 768, 2,304
or 3,864 doubles per vertex or cell, respectively, where we
can run 1, 2, 4, \ldots, 1024 floating point operations (FLOPS) per
double.
For 1 and 2 FLOPS per double, our arithmetic load mirrors the Stream
SCALE/Stream TRIAD benchmark \cite{McCalpin:95:Stream}.
Other work-per-byte configurations resemble characteristic application
profiles:
Two unknowns per vertex have to be stored at least for any matrix-free equation
system solve.
They hold the right-hand side and the solution which yields between 32
and 128 flops per double for a cell-wise matrix-vector product.
If we store low-order discretization stencils per vertex, the memory footprint
grows to at least 11 doubles per vertex (9 for the stencil for $d=2$ plus the two
unknowns) or 28 for $d=3$ if we have an analytic right-hand side.
Patches within the spacetree can yield any memory footprint per grid entity, but
768 unknowns per cell or vertex, respectively, are a reasonable ``small'' count.
It arises for example from the shallow water code
\cite{Weinzierl:14:BlockFusion} with $16\times 16$ patches and three unknowns (velocity plus water height).
%embedded into the spacetree's fine grid cells.
Lattice Boltzmann with D2Q9 using $16 \times 16$
subgrids at the same time yields 2304 unknowns, while D3Q19 yields 3864
\cite{Neumann:13:Diss}.
 
